ACRIC: Securing Legacy Communication Networks via Authenticated Cyclic Redundancy Integrity Check

The increasing integration of modern IT technologies into OT technologies and industrial systems is expanding the vulnerability surface of legacy infrastructures, which often rely on outdated protocols and resource-constrained devices. Recent security incidents in safety-critical industries exposed how the lack of proper message authentication enables attackers to inject malicious commands or alter system behavior, revealing fundamental security weaknesses in existing architectures. These shortcomings have thus prompted new regulations that emphasize the pressing need to strengthen cybersecurity, particularly in legacy systems. Authentication is widely recognized as a fundamental security measure that enhances system resilience. However, its adoption in legacy industrial environments is limited due to practical challenges like backward compatibility, message format changes, and hardware replacement or upgrades costs. In this paper, we introduce ACRIC, a message authentication solution to secure legacy industrial communications explicitly tailored to overcome those challenges all at once. ACRIC uniquely leverages cryptographic computations applied to the CRC field - already present in most industrial communication protocols - ensuring robust message integrity protection and authentication without requiring additional hardware or modifications to existing message formats. ACRIC's backward compatibility and protocol-agnostic nature enable coexistence with non-secured devices, thus facilitating gradual security upgrades in legacy infrastructures. Formal security assessment and experimental evaluation on an industrial-grade testbed demonstrate that ACRIC provides robust security guarantees with minimal computational overhead (~ 4 us). These results underscore ACRIC's practicality, cost-effectiveness, and suitability for effective adoption in resource-constrained industrial environments.

==> OLD_texts.tex <==
\subsection{Hash-Chain Management}\label{sec:ChainManagement}
Hash values — and consequently hash chains — are fundamental for ensuring the security of \ac{acric}.
They serve as secret keys for \ac{otp} encryption, preventing attackers from deducing the secret \ac{iv} used in \ac{crc} computations.
However, managing hash chains in memory-constrained devices, particularly within large networks, can be challenging.
Efficient hash chain management is therefore critical to balance memory usage, computational overhead, and security.
In this section, we discuss strategies for managing hash chains, outlining their constraints, benefits, and trade-offs.
Tables~\ref{tab:HashChain} and~\ref{tab:HashChainComputation} summarize our findings.\\
\indent \textbf{\underline{Hash Chain Consumption.}}
Hash chain consumption describes how individual hash values are utilized within a chain.
In a \textbf{Backward Consumption} strategy, hash values are consumed in reverse order, starting from the tail \(h_n\) and moving backward to the root \(h_0\).
Due to the pre-image resistance property, exposing a hash \(h_i\) does not allow an attacker to derive previous values \(h_j\) for \(j < i\) \cite{hash-review}.
However, this strategy requires pre-computation and storage of the entire chain, increasing memory demands.
With a \textbf{Forward Consumption} approach, hash values are instead sequentially consumed from the root \(h_0\) to the tail \(h_n\).
This strategy avoids pre-computing the full chain, significantly reducing memory usage.
However, without additional protection, exposure of a hash \(h_i\) allows attackers to compute subsequent hashes \(h_j \;, \forall \, j > i\).
To prevent this, the hashing process must incorporate a secret key, ensuring that subsequent hash values remain secure even if an earlier value is compromised.\\
\indent \textbf{\underline{Hash Chain Storage.}}
Hash chain storage refers to how hash chains are allocated, stored, and synchronized among devices.
By following an \textbf{entity-based} storage, the device maintains its hash chain to authenticate the messages it transmits.
This approach presents two main limitations.
First, it requires device identifiers to be included in message payloads, which some protocols (e.g., CAN-bus~\cite{CAN}) do not inherently support, especially for broadcast communications.
Second, receiving devices must track the hash index to correctly verify the incoming messages.
Managing indices either demands constant monitoring of all transmissions or adding an index parameter to each message, thus reducing data throughput.
On the other hand, with a \textbf{pair-based or group-based} storage, each pair of nodes or device group shares a dedicated hash chain.
Pair-based storage assigns a unique chain to each pair of devices, while group-based storage uses a shared chain among group members for broadcast scenarios.
Unlike entity-based storage, these approaches simplify synchronization between senders and receivers, eliminating the need for explicit hash indexing.
Table~\ref{tab:HashChain} analyzes storage overhead for both storage strategies in combination with chain consumption methods.
From this analysis, we conclude that the \textit{forward-consumption pair-based} strategy offers the lowest storage overhead, making it particularly suitable for legacy and resource-constrained environments.
\input{Tables/HashChain}

\indent \textbf{\underline{Hash Chain Computation.}}
Hash chain computation strategies significantly impact system performance and security.
We identify three possible strategies.
With a \textbf{runtime computation} strategy, hash values are generated as needed during system operation.
This ensures freshness and limits exposure to pre-computation attacks, requiring minimal memory.
However, it increases computational demands, potentially introducing latency due to real-time cryptographic processing.
In an \textbf{offline computation} strategy, the entire hash chain is computed before deployment.
This minimizes runtime computational demands but significantly increases memory requirements since the entire chain must be stored.
Finally, the \textbf{hybrid strategy} combines aspects of both runtime and offline approaches. 
A portion of the chain is pre-computed and stored, while the remainder is computed as needed during operation.
This balances reduced memory usage with lower computational load, achieving an optimal trade-off between system efficiency and security.
Table~\ref{tab:HashChainComputation} summarizes each computation strategy, detailing their advantages, drawbacks, and compatibility with chain consumption methods.

\input{Tables/HashChainComputation}

==> Tables/Collision_probabilities.tex <==
%---------------------
% \begin{table*}[]
% \renewcommand{\arraystretch}{1.25}
% \centering
% \caption{\textcolor{red}{CAPTION}}
% \label{tab:CollisionProb}
% \resizebox{0.6\linewidth}{!}{%
% \begin{tabular}{|l|c|c|}
% \hline
% \multicolumn{1}{|c|}{
%     \textbf{\begin{tabular}[c]{@{}c@{}}CRC\\ Algorithm\end{tabular}}} &
%     %\textbf{\begin{tabular}[c]{@{}c@{}}CRC bit-length\\ (n)\end{tabular}} &
%     \textbf{\begin{tabular}[c]{@{}c@{}}Is Injective\\ (m = 1)\end{tabular}} &
%     \textbf{\begin{tabular}[c]{@{}c@{}}Collision Probability\\ \(P_c\)\end{tabular}} \\ \hline
    
% Theoretical (n-bits)                     & N.A.    & \(\frac{m-1}{2^n - 1} + \frac{2^n - m}{\left(2^n-1\right)^2}\) \\ \hline
% CRC-8                                    & \ccmark & \(2^{-8}\) \\
% CRC-8/CDMA2000                           & \ccmark & \(2^{-8}\) \\
% CRC-8/ITU                                & \ccmark & \(2^{-8}\) \\ \hline
% CRC-16/CCITT-FALSE                       & \ccmark & \(2^{-16}\) \\
% CRC-16/ANSI (DNP)                        & \ccmark & \(2^{-16}\) \\
% CRC-16/MODBUS                            & \ccmark & \(2^{-16}\) \\ \hline
% CRC-32                                   & \ccmark & \(2^{-32}\) \\
% CRC-32C                                  & \ccmark & \(2^{-32}\) \\
% CRC-32Q                                  & \ccmark & \(2^{-32}\) \\ \hline
% \end{tabular}
% }
% \end{table*}
%------------------


\begin{table*}[]
\renewcommand{\arraystretch}{1.25}
\centering
\caption{\ac{acric}'s collision probabilities with different \ac{crc} functions. For security, while injectivity is desirable, linearity is not.}
\label{tab:CollisionProb}
\resizebox{0.65\linewidth}{!}{%
\begin{tabular}{|l|c|c|c|}
\hline
\rowcolor{gray!15}
\multicolumn{1}{|c|}{
    \textbf{\begin{tabular}[c]{@{}c@{}}CRC\\ Algorithm\end{tabular}}} &
    \textbf{\begin{tabular}[c]{@{}c@{}}Is Injective\\ (m = 1)\end{tabular}} &
    \textbf{Is linear}  &
    \textbf{\begin{tabular}[c]{@{}c@{}}Collision \\ Probability\end{tabular}} \\ \hline
    
Theoretical (n-bits)  & N.A.                        & N.A.                      & \(\frac{m-1}{2^n - 1} + \frac{2^n - m}{\left(2^n-1\right)^2}\) \\ \hline
CRC-8                 & \multirow{3}{*}{\ccmark}    & \multirow{3}{*}{\xxmark}  & \multirow{3}{*}{\(2^{-8}\)}            \\
CRC-8/CDMA2000        &                             &                           &            \\
CRC-8/ITU             &                             &                           &            \\ \hline
CRC-16/CCITT-FALSE    & \multirow{3}{*}{\ccmark}    & \multirow{3}{*}{\xxmark}  & \multirow{3}{*}{\(2^{-16}\)}           \\
CRC-16/ANSI (DNP)     &                             &                           &            \\
CRC-16/MODBUS         &                             &                           &            \\ \hline
CRC-32                & \multirow{3}{*}{\ccmark}    & \multirow{3}{*}{\xxmark}  & \multirow{3}{*}{\(2^{-32}\)}           \\
CRC-32C               &                             &                           &            \\
CRC-32Q               &                             &                           &            \\ \hline
\end{tabular}%
}
\end{table*}

==> Tables/HashChain.tex <==
\begin{table}[!h]
\renewcommand{\arraystretch}{1.2}
\centering
\caption{Storage overhead of hash chain consumption strategies.
\(x\): the number of bits of a single hash value; \(n\_hash\): the number of hash values in the chain; \(N\): the number of network nodes (\ac{p2p}) or groups (broadcast) a node is part of.
}
\label{tab:HashChain}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|cl|l|l|l|}
\hline

\multicolumn{2}{|c|}{\textbf{Hash Chain Consumption}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Storage Approach}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Saved Values}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Storage Overhead\\ (bits)\end{tabular}}}} \\ \cline{1-2}
\multicolumn{1}{|c|}{\textbf{Approach}} & 
\multicolumn{1}{c|}{\textbf{Constraints}} & 
\multicolumn{1}{c|}{} & 
\multicolumn{1}{c|}{} & 
\multicolumn{1}{c|}{} \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textit{Backward}}} &
  \multirow{3}{*}{\begin{tabular}[c]{c@{}c@{}}Compute and store entire\\chain in advance \end{tabular} } &
  \textit{Entity-based} &
    \begin{tabular}[c]{@{}l@{}}
        1 full own hash chain \\
        N-1 receivers' single hash values
   \end{tabular} &  
  \multicolumn{1}{c|}{\(x * (n\_hash + N -1)\)} \\ \cline{3-5} 
\multicolumn{1}{|c|}{} &
   &
  \textit{Pair / Group-based} &
  \begin{tabular}[c]{@{}l@{}}
        \ac{p2p}: N-1 full hash chains\\
        Broadcast: N full hash chains
  \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}
        \ac{p2p}: \((N-1)* n\_hash * x\) \\
        Broadcast: \(N * n\_hash * x\)
  \end{tabular} \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textit{Forward}}} &
  \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{c@{}c@{}}Secret key as part \\ of input required\end{tabular}}} &
  \textit{Entity-based} &
  \begin{tabular}[c]{@{}l@{}}
        1 single own hash value\\
        N-1 receivers' single hash values
  \end{tabular} &
  \multicolumn{1}{c|}{\(N * x\)} \\ \cline{3-5} 
\multicolumn{1}{|c|}{} &
   &
  \textit{Pair / Group-based} &
  \begin{tabular}[c]{@{}l@{}}
        \ac{p2p}: N-1 single hash values\\
        Broadcast: N single hash values
  \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}
        \ac{p2p}: \((N-1) * x\) \\
        Broadcast: \(N * x\)
  \end{tabular} \\ \hline
\end{tabular}
}
\end{table}

==> Tables/HashChainComputation.tex <==
\begin{table}[!h]
\renewcommand{\arraystretch}{1.2}
\centering
\caption{Hash chain computation approaches comparison.}
\label{tab:HashChainComputation}
\resizebox{0.69\linewidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
\rowcolor{gray!15}
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Computation\\Approach\end{tabular}}} &
 \multicolumn{1}{c|}{\textbf{Pros (\textcolor{green}{\ccmark}) \& Cons (\textcolor{red}{\xmark})}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Chain \\ consumption
  \end{tabular}}} \\
  \hline
  
\multicolumn{1}{|c|}{\textit{Runtime}} &
  \begin{tabular}[c]{@{}l@{}}
    \([\)\textcolor{green}{\ccmark}\(]\) Minimum memory overhead \\
    \([\)\textcolor{red}{\xmark}\(]\) Introduces transmission delay 
  \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}
    \([\)\ccmark\(]\) Forward \\
    \([\)\xmark\(]\) Backward
  \end{tabular} \\
  \hline
    
\multicolumn{1}{|c|}{\textit{Offline}} &
   \begin{tabular}[c]{@{}l@{}}
      \([\)\textcolor{green}{\ccmark}\(]\) No transmission delay\\
      \([\)\textcolor{red}{\xmark}\(]\) Lager memory overhead
   \end{tabular}&
  \begin{tabular}[c]{@{}l@{}}
    \([\)\ccmark\(]\) Forward\\
    \([\)\ccmark\(]\) Backward
  \end{tabular}\\
  \hline

\multicolumn{1}{|c|}{\textit{Hybrid}} &
  \begin{tabular}[c]{@{}l@{}}
    \([\)\textcolor{green}{\ccmark}\(]\) No transmission delay\\
    \([\)\textcolor{green}{\ccmark}\(]\) Smaller memory overhead w.r.t. offline\\
    \([\)\textcolor{red}{\xmark}\(]\) Larger memory overhead w.r.t. runtime
  \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}
    \([\)\ccmark\(]\) Forward \\
    \([\)\ccmark\(]\) Backward
  \end{tabular} \\ \hline
\end{tabular}%
}
\end{table}
